MoPS: Modular Story Premise Synthesis for Open-Ended Automatic Story Generation

A story premise succinctly defines a story's main idea, foundation, and trajectory. It serves as the initial trigger in automatic story generation. Existing sources of story premises are limited by a lack of diversity, uneven quality, and high costs that make them difficult to scale. In response, we introduce Modular Story Premise Synthesis (MoPS) which breaks down story premises into modules like background and persona for automated design and generation. MoPS consists of three phases: (1) Precollect a consistent set of candidates for each module to form a nested dictionary. (2) Extract a key path from the nested dictionary as the premise design. (3) Instruct an LLM to integrate the design into a coherent premise sentence. Thorough evaluations demonstrate that our synthesized premises excel in diversity, fascination, completeness, and originality compared to those induced from large language models and captured from public story datasets. Similarly, the extended novels and scripts generated from our premises also exhibit higher quality. In supplementary materials, we provide the MoPS code suite, along with 7.6k generated premises and 1k extended stories. Code: https://github.com/GAIR-NLP/MoPS.

==> tables/motivation_example.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \begin{tabularx}{\textwidth}{>{\columncolor{rowcolor1}}X|>{\columncolor{rowcolor2}}X} 
    \toprule
    {\keyword{\textbf{Premise A:}} \textit{\small A powerful Roman general,\textcolor{my_green}{\uline{granted immortality by a vengeful deity}}, must choose between loyalty to the empire and leading a rebellion, ultimately decide to bring justice and equality to the corrupt rulers of the Roman Empire. }} & {\keyword{\textbf{Premise B:}} \textit{A Roman general chooses between loyalty to empire and leading a rebellion for justice and equality. }} \\

    \midrule

    \vspace{0.1cm}
    \keyword{\textbf{Poster A:}} 
    \qquad\quad\adjustbox{width=0.15\textwidth,valign=c}{\includegraphics{figures/poster1.png}}
    \newline
    \vspace{0.2cm}
    
    \keyword{\textbf{Story A:}} Centuries ago, in the heart of ancient Rome, there was a powerful general named Lucius, \greenunline{who had been granted immortality by a vengeful deity}. As the empire crumbled under the weight of corruption and tyranny, Lucius faced a fateful decision: remain loyal to the empire that had once revered him, or lead a rebellion to bring justice and equality to its corrupt rulers. After witnessing the suffering of the oppressed, Lucius chose to forsake his loyalty to the empire, \greenunline{vowing to use his immortality to dismantle the corrupt regime}. With unwavering determination, he rallied the oppressed citizens, becoming a symbol of hope and change. Together, they waged a relentless battle for a brighter future, where justice and equality would reign, and the legacy of Lucius would live on through the ages as \greenunline{a beacon of righteous rebellion against tyranny}.
    &
    \vspace{0.1cm}
    \keyword{\textbf{Poster B:}} 
    \qquad\quad\adjustbox{width=0.15\textwidth,valign=c}{\includegraphics{figures/poster2.png}}
    \newline
    \vspace{0.2cm}
    
    \keyword{\textbf{Story B:}} In the heart of the Roman Empire, General Lucius found himself \redunline{torn between two irreconcilable paths}. On one hand, he had sworn an oath of unwavering loyalty to the empire that had granted him power and prestige. On the other, he witnessed the relentless oppression and suffering of the common people, burdened by heavy taxes and brutal tyranny. \redunline{The call for justice and equality} resonated within him like a thunderous battle drum. In a moment of agonizing decision, he chose to forsake his allegiance to the empire, forsaking his name and status to lead a rebellion for the oppressed, determined to wield his military prowess to carve a path toward a more just and equitable future.
    \\
    \midrule
    \rowcolor{shadecolor}
    \multicolumn{2}{>{\arraybackslash}p{\dimexpr\linewidth-2\tabcolsep}}{
    \keyword{\textbf{Review by GPT4:}}
    Story $A$ is better than $B$.
    
    Story $A$ is written with \greenunline{a more vivid and immersive narrative style}.
    It provides greater detail about \greenunline{the protagonist's character, motivations, and the historical context}. 
    Phrases like "vowed to use his immortality to dismantle the corrupt regime" and "a beacon of righteous rebellion against tyranny" \greenunline{add a mythical and heroic dimension to the protagonist, Lucius}.
    The mention of a vengeful deity granting immortality to Lucius \greenunline{adds a layer of mythological intrigue and depth to his character}.
    Furthermore, the depiction of the empire's corruption and Lucius's transition from loyalty to rebellion is \greenunline{more dramatically and emotionally engaging, enhancing the reader's investment in the story}.
    
    Story $B$, while also well-written, \redunline{lacks the same level of detail} and \redunline{narrative flair}. It presents \redunline{a more straightforward account} of Lucius's dilemma and decision. The story \redunline{misses opportunities to deepen the character development and historical context}, resulting in a narrative that \redunline{feels less engaging and impactful} compared to $A$.
    Additionally, $B$ \redunline{repeats certain ideas}, such as Lucius being torn between loyalty and justice, which can \redunline{make the plot feel slightly redundant}.
    } \\
    \bottomrule
    \end{tabularx}
    \caption{
    Motivation example of the significance of story premises.
    %
    $A$ represents a story premise synthesized by MoPS, while $B$ is a manually simplified version of $A$.
    %
    Story premises serve as prompts to instruct \texttt{Dall-E} and \texttt{chatgpt} to generate posters and short stories.
    %
    The review by \texttt{gpt-4} underscores the importance of a story premise in crafting engaging narratives.}
    \vspace{-0.5cm}
    \label{tab:motivation}
\end{table*}

==> tables/premise_ablation.tex <==
\begin{table}[htbp]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
& Fascination$\uparrow$ & Completeness$\uparrow$ & Originality$\uparrow$ \\ \midrule
MoPS                      &  \textbf{75.81}           &  \textbf{75.10}            & \underline{59.90}           \\  \midrule
m/f Twist                      &  \underline{74.56}           &  \underline{73.20}            &  41.90           \\
m/f Ending                      & 74.43           & 71.40            &  42.70           \\
m/f Event                      &  74.16           &  67.20            &  39.10           \\ 
m/f Persona                      & 73.30           &  57.25            &   26.90           \\  \midrule
w/o Dependence                      &  65.77          & 65.75            &  \textbf{74.51}           \\
\bottomrule
\end{tabular}}
\caption{Ablation results. m/f -> ``mask all components following a certain component''. w/o -> `` without''.} %The optimal values with $p$ < 0.05 for each column are \textbf{bolded}, and the second-best  values with $p$ < 0.05 are \underline{underlined}.}
\label{tab:ablation_scores}
\end{table}

==> tables/premise_score.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{Tokens} & \multicolumn{2}{c}{Diversity Score} & \multicolumn{4}{c}{Quality Score (mean $\pm$ std)} \\ \cmidrule(l){3-4} \cmidrule(l){5-8} 
                     &                         & Breadth$\uparrow$          & Density$\downarrow$           & Fascination$\uparrow$ & Completeness$\uparrow$ & Originality$\uparrow$ & Average$\uparrow$ \\ \midrule
MoPS  &  50.24 & \textbf{3545.78} & \textbf{7.52} & \textbf{75.66} $\pm$ 3.98 & \textbf{74.78} $\pm$ 3.16 & \underline{60.01} $\pm$ 23.61 & \textbf{70.15} $\pm$ 10.25
 \\
CPX  & 45.22 & 2618.18 &  14.63 &  73.96 $\pm$ 3.95 & \underline{70.88} $\pm$ 6.33 & 26.60 $\pm$ 12.94 & 57.15 $\pm$ 7.74~~ \\
VIL  & 37.61 & \underline{3050.72} & 11.08 &  71.50 $\pm$ 5.95  & ~~53.66 $\pm$ 13.20 
 &  20.82 $\pm$ 11.71 & 48.66 $\pm$ 10.29\\
DOC  & 45.81 & 1901.04 & 14.22 & \underline{74.33} $\pm$ 6.31 &  ~~69.87 $\pm$ 11.80 &  50.65 $\pm$ 27.57 &  64.95 $\pm$ 15.23\\
WP  & 42.54  & 3013.61 & \underline{8.53} & ~~\underline{74.49} $\pm$ 13.65 &  ~~43.57 $\pm$ 17.46  & \textbf{71.05} $\pm$ 30.18 & 63.04 $\pm$ 20.43\\
STM  & 77.78 & 1918.67 & 13.82 & ~~\textbf{75.83} $\pm$ 10.79 &  ~~66.45 $\pm$ 16.30 &  \underline{61.51} $\pm$ 30.62 & \underline{67.93} $\pm$ 19.24\\
\bottomrule
\end{tabular}}
\caption{Diversity score and quality score of story premises.
%
The plots for diversity scores are in Fig.~\ref{fig:breadth_score},~\ref{fig:density_score}, while the distribution plots for quality scores are in Fig.~\ref{fig:fascination_score},~\ref{fig:completeness_score},~\ref{fig:originality_score}.
%
The optimal values (with $p$ < 0.05) will be \textbf{bolded}, and the second-best values (with $p$ < 0.05) will be \underline{underlined}.
}
\label{tab:premise_scores}
\vspace{-5pt}
\end{table*}

==> tables/story_score.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lccc@{}}
    \toprule
    & Fascination$\uparrow$ & Completeness$\uparrow$ & Originality$\uparrow$ \\ \midrule
    MoPS-RecurrentGPT   & \textbf{74.60} & \textbf{60.30} & \underline{69.45}\\
    CPX-RecurrentGPT  &  \textbf{74.20} & \underline{56.05} & 45.60\\
    VIL-RecurrentGPT  &  \textbf{74.40} & \textbf{57.30} &  48.00\\
    DOC-RecurrentGPT  &  \underline{73.30} &  \textbf{57.60} &  \underline{66.75}\\
    WP-RecurrentGPT  & \textbf{74.40}&  55.45 & \textbf{81.15}\\
    STM-RecurrentGPT & 73.00 &  54.95 &  \underline{64.20}\\ \midrule
    MoPS-Dramatron  & \textbf{70.59} & \textbf{74.50} & \textbf{94.20} \\
    CPX-Dramatron  &  \textbf{70.24} & \textbf{74.50} & \textbf{92.60} \\
    VIL-Dramatron  &  \underline{67.92} & \textbf{74.30} &  \underline{83.50} \\
    DOC-Dramatron  &  \textbf{70.35} &  \textbf{74.00} &  \textbf{91.35}\\
    WP-Dramatron  & 62.90 &  62.95 & \textbf{92.35} \\
    STM-Dramatron  & \underline{68.29} &  \underline{70.40} &  \underline{84.80}\\
    \bottomrule
    \end{tabular}}
    \caption{Quality Score of premise-based stories. The optimal values (with $p$ < 0.05) will be \textbf{bolded}, and the second-best values (with $p$ < 0.05) will be \underline{underlined}.}
    \label{tab:story_score}
    \end{table}
